The filamentary structures in the CO emission toward the Milky Way disk

We present a statistical study of the filamentary structure orientation in the CO emission observations obtained in the Milky Way Imaging Scroll Painting (MWISP) survey in the range $25.8\deg < l < 49.7\deg$, $|b| \leq 1.25\deg$, and $-100 < v_{\rm LSR} < 135$ km/s. We found that most of the filamentary structures in the $^{12}$CO and $^{13}$CO emission do not show a global preferential orientation either parallel or perpendicular to the Galactic plane. However, we found ranges in Galactic longitude and radial velocity where the $^{12}$CO and $^{13}$CO filamentary structures are parallel to the Galactic plane. These preferential orientations are different from those found for the HI emission. We consider this an indication that the molecular structures do not simply inherit these properties from parental atomic clouds. Instead, they are shaped by local physical conditions, such as stellar feedback, magnetic fields, and Galactic spiral shocks.

==> PlanckTable.tex <==
%Planck table template file, to be used with A&A style and Planck.tex to produce Planck tables %  for publication.
%
% version 11 September 2011 ---  CRL

\begin{table*}[tmb]                 % table* is a two-column table.  Drop the * for one column.
\begingroup
\newdimen\tblskip \tblskip=5pt
\caption{}                          % Caption goes here.
\label{}                            % Label goes here.
\nointerlineskip
\vskip -3mm
\footnotesize
\setbox\tablebox=\vbox{
   \newdimen\digitwidth 
   \setbox0=\hbox{\rm 0} 
   \digitwidth=\wd0 
   \catcode`*=\active 
   \def*{\kern\digitwidth}
%
   \newdimen\signwidth 
   \setbox0=\hbox{+} 
   \signwidth=\wd0 
   \catcode`!=\active 
   \def!{\kern\signwidth}
%
\halign{                            % Template goes here.
\noalign{\doubleline}
                                    % Table headings go here.
\noalign{\vskip 3pt\hrule\vskip 5pt}
                                    % Body of table goes here.
\noalign{\vskip 5pt\hrule\vskip 3pt}}}
%\endPlancktable                    % ends one-column \halign
\endPlancktablewide                 % ends two-column \halign
\tablenote a Footnote a.\par
\tablenote b Footnote b.\par
\endgroup
\end{table*}                        % table* is a two-column table.  Drop the * for one column.


==> polar_definitions.tex <==
%This is a proposal for homogeneous polarization notations in the
%Planck PIP papers.
% They are the same as in Fig 14 of the paper by Levrier, except for B
%Feel free to add to it if you need more, or propose for changes.
%JPB Jan 21 2013

%=== Stokes parameters
\newcommand{\StokesI}{\rm I}                    %Intensity
\newcommand{\StokesQ}{\rm Q}                    %Q
\newcommand{\StokesU}{\rm U}                    %U
%=== Polarization quantities
\newcommand{\polint}{\rm P}                     %polarization intensity
\newcommand{\polfrac}{\rm p}                    %polarization fraction
\newcommand{\polang}{\rm \psi}                  %polarization angle
\newcommand{\sigpolfrac}{\rm \sigma_{\polfrac}}   %polarization fraction uncertainty
\newcommand{\sigpolang}{\rm \sigma_{\polang}}     %polarization angle uncertainty
\newcommand{\polangsky}{\rm \gamma}             %B-field angle wrt sky plane
\newcommand{\DeltaAng}{\Delta \polang}          %polarization angle structure function
%=== Stockes parameters variances
\newcommand{\sigII}{\rm \sigma_{II}}            % Intensity sqrt(variance)
\newcommand{\sigQQ}{\rm \sigma_{QQ}}            % Q sqrt(variance)
\newcommand{\sigUU}{\rm \sigma_{UU}}            % U sqrt(variance)
\newcommand{\sigIQ}{\rm \sigma_{IQ}}            % IQ sqrt(covariance)
\newcommand{\sigIU}{\rm \sigma_{IU}}            % IU sqrt(covariance)
\newcommand{\sigQU}{\rm \sigma_{QU}}            % QU sqrt(covariance)
\newcommand{\sigsquareII}{\rm \sigma^2_{II}}    % Intensity variance
\newcommand{\sigsquareQQ}{\rm \sigma^2_{QQ}}    % Q variance
\newcommand{\sigsquareUU}{\rm \sigma^2_{UU}}    % U variance
\newcommand{\sigsquareIQ}{\rm \sigma^2_{IQ}}    % IQ covariance
\newcommand{\sigsquareIU}{\rm \sigma^2_{IU}}    % IU covariance
\newcommand{\sigsquareQU}{\rm \sigma^2_{QU}}    % QU covariance
%=== B field
\newcommand{\Borth}{\rm B_{\perp}}              %B orthogonal to LOS (ie, Plane of sky)
\newcommand{\Bpar}{\rm B_{\parallel}}           %B parallel to LOS


